A Variational-Sequential Graph Autoencoder for Neural Architecture Performance Prediction

In computer vision research, the process of automating architecture engineering, Neural Architecture Search (NAS), has gained substantial interest. In the past, NAS was hardly accessible to researchers without access to large-scale compute systems, due to very long compute times for the recurrent search and evaluation of new candidate architectures. The NAS-Bench-101 dataset facilitates a paradigm change towards classical methods such as supervised learning to evaluate neural architectures. In this paper, we propose a graph encoder built upon Graph Neural Networks (GNN). We demonstrate the effectiveness of the proposed encoder on NAS performance prediction for seen architecture types as well an unseen ones (i.e., zero shot prediction). We also provide a new variational-sequential graph autoencoder (VS-GAE) based on the proposed graph encoder. The VS-GAE is specialized on encoding and decoding graphs of varying length utilizing GNNs. Experiments on different sampling methods show that the embedding space learned by our VS-GAE increases the stability on the accuracy prediction task.

==> exp_sampling.tex <==
\color{Plum}

In this experiment we use the different sampling methods from Section \ref{sec:sampling} to downsize the training set with different factors ranging from $1\%$ to $90\%$ of the original size. We keep the validation set and the test set unchanged and calculate the test error regarding the best validation error over $100$ epochs. The results are outlined in Figure \ref{fig:sampling}. While the error fluctuates drastically for the sampling methods in the discrete space, the latent space created by VS-GAE enables a sampling method that is way more stable. Interestingly, we cannot confirm that sampling uniformly by means of the edit
distance gives any stability advantage over sampling uniformly at random.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/sampling.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/sampling_10.pdf}
    \end{subfigure}
    \caption{The test error regarding sample method and sample size visualized in two different resolutions.}\label{fig:sampling}
\end{figure}

\color{blue}

==> related_work_VAE.tex <==
Variational autoencoders (VAE) \cite{Kingma2014} allow to learn a recognition model $q_{\phi}(\textbf{z} \vert G)$, i.e. the encoder, and a generative model $p_{\theta}(G \vert \textbf{z})$, i.e. the decoder, jointly, where $\phi$ and $\theta$ are the outputs of the encoder and decoder, respectively. Note, the VAE learns the parameters of the data's probability distribution instead of a lower dimensional representation of the input data. \\
The VAE learns by maximizing a lower bound estimator on the log-likelihood $\text{log } p_{\theta}(G)$:
\begin{eqnarray}\label{VAE}
{\mathcal{L}}(\theta, \phi ; G) &=& \mathbb{E}_{q_{\phi}(\textbf{z} \vert  G)} \big[\log p_{\theta}(G \vert \textbf{z}) \big]  \nonumber \\
&-& \text{D}_{\text{KL}} (q_{\phi}(\textbf{z} \vert G) \Vert p_{\theta}(\textbf{z}))
\end{eqnarray}	
From the trained VAE model new data can be generated by sampling $\textbf{z} \sim p_{\theta}(\textbf{z})$ and decode it by means of $p_{\theta}(G \vert \textbf{z})$. 


% Given a  dataset $X=\{x^{(i)}\}^N_{i=1}$ with $N$ i.i.d. discrete  data $x$, generating new data is a random process. First an unobserved continuous random variable $z^{(i)}$ is generated from the prior distribution $p_{\theta^*}(\textbf{z})$. Second a value $x^{(i)}$ is generated from some posterior distribution $p_{\theta^*}(\textbf{x} \vert \textbf{z})$, with $\theta$ being some generative model parameters. 
% Since the posterior $p_{\theta}(z \vert x)$ cannot be guaranteed to be tractable, the authors propose a recognition model $q_{\phi}(z \vert x) \approx p_{\theta}(z \vert x)$, with the recognition model parameters $\phi$ are learned jointly with the generative model parameters $\theta$. 
% The VAE learns by maximizing a lower bound estimator
% \begin{eqnarray}\label{VAE}
% {\mathcal{L}}(\theta, \phi ; x^{(i)}) &=& \mathbb{E}_{q_{\phi}(\textbf{z} \vert x^{(i)})} \big[\text{log ~} p_{\theta}(x^{(i)} \vert \textbf{z}) \big]  \nonumber \\
% &-& \text{D}_{\text{KL}} (q_{\phi}(\textbf{z} \vert x^{(i)}) \Vert p_{\theta}(\textbf{z}))
% \end{eqnarray}	
% The first term  of eq.  (\ref{VAE}) is known as the expected negative reconstruction error, where the function $g_{\phi}(\cdot)$ is chosen s.t. it maps a datapoint $x^{(i)}$ and a random noise vector $\varepsilon^{(l)}$ to a sample from the approximated posterior $q_{\phi}(\textbf{z} \vert \textbf{x})$. The second term of eq. (\ref{VAE}) is the Kullback-Leibler Divergence, which acts as a regularizer for $\phi$, encouraging the approximate posterior to be close to the prior.  

% When considering neural networks as encoder and decoder, \cite{Kingma2014} set the assumptions of the prior being $p_{\theta}(\textbf{z}) \sim \mathcal{N}(\textbf{z};0, \mathbbm{1})$ and the likelihood $p_{\theta}(\textbf{x}\vert \textbf{z}) \sim \mathcal{N}(\mu, \Sigma)$. Since the true posterior $p_{\theta}(\textbf{z} \vert \textbf{x})$ is intractable, the authors set $$\text{log~}q_{\phi}(\textbf{z} \vert x^{(i)}) = \log~ \mathcal{N}(\textbf{z};\mu^{(i)}, \sigma^{2(i)} \mathbbm{1})$$ , i.e.the approximate posterior is a multivariate Gaussian distribution with diagonal covariance structure, with $\mu^{(i)}$ and $\sigma^{(i)}$ being outputs of the encoding. 
% To sample a latent variable from the prior, the authors use $z^{(i,l)}=g_{\phi}(x^{(i)}, \varepsilon^{(l)}) = \mu^{(i)} + \sigma^{(i)} \odot \varepsilon^ {(l)}$, with $\varepsilon^{(l)} \sim \mathcal{N}(0, \mathbbm{1})$.


==> related_work_nas.tex <==
Neural Architecture Search (NAS) \cite{Zoph2017, Real2017, Zoph2018, Liu2018, Pham2018}, the process of designing neural network architectures in an automatic way, gained substantial attention recently. See \cite{Elsken2019} for an overview and detailed survey over recent NAS methods. The currently most successful approaches follow different paradigms: Reinforcement learning (RL) \cite{Zoph2017, Zoph2018,Pham2018} as a NAS strategy considers the neural architecture generation as the agent's action with it's reward given in terms of validation accuracy. Evolutionary Algorithm (EA) \cite{Real2017, Liu2017} approaches optimize the neural architectures themselves by guiding the mutation of architectures and evaluating their fitness given in terms of validation accuracy. Bayesian optimization (BO) \cite{Kandasamy2018} derive kernels for architecture similarity measurements to extrapolate the search space. Gradient based methods \cite{Liu2018, Luo2018} use continuous relaxations of neural architectures to allow for gradient-based optimization. 


